Mitigating Spatial Error in the iterative-Quasi-Monte Carlo (iQMC) Method for Neutron Transport Simulations with Linear Discontinuous Source Tilting and Effective Scattering and Fission Rate Tallies

The iterative Quasi-Monte Carlo (iQMC) method is a recently proposed method for multigroup neutron transport simulations. iQMC can be viewed as a hybrid between deterministic iterative techniques, Monte Carlo simulation, and Quasi-Monte Carlo techniques. iQMC holds several algorithmic characteristics that make it desirable for high performance computing environments including a $O(N^{-1})$ convergence scheme, ray tracing transport sweep, and highly parallelizable nature similar to analog Monte Carlo. While there are many potential advantages of using iQMC there are also inherent disadvantages, namely the spatial discretization error introduced from the use of a mesh across the domain. This work introduces two significant modifications to iQMC to help reduce the spatial discretization error. The first is an effective source transport sweep, whereby the source strength is updated on-the-fly via an additional tally. This version of the transport sweep is essentially agnostic to the mesh, material, and geometry. The second is the addition of a history-based linear discontinuous source tilting method. Traditionally, iQMC utilizes a piecewise-constant source in each cell of the mesh. However, through the proposed source tilting technique iQMC can utilize a piecewise-linear source in each cell and reduce spatial error without refining the mesh. Numerical results are presented from the 2D C5G7 and Takeda-1 k-eigenvalue benchmark problems. Results show that the history-based source tilting significantly reduces error in global tallies and the eigenvalue solution in both benchmarks. Through the effective source transport sweep and linear source tilting iQMC was able to converge the eigenvalue from the 2D C5G7 problem to less than $0.04\%$ error on a uniform Cartesian mesh with only $204\times204$ cells.

==> tables/c5g7_results_fast.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{table}
\caption{Region averaged scalar flux from 2D-C5G7: groups 1-2 (fast)}
\centering
\begin{tabular}{|lcccccc|}
\hline
\textbf{Mesh} & \textbf{Method} & \textbf{I} & \textbf{II} & \textbf{III} & \textbf{IV} & \textbf{Moderator} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c}{\cellcolor[HTML]{EFEFEF}Coarse} &
  \begin{tabular}[c]{@{}c@{}}Monte Carlo \\ (Reference) \end{tabular}&
  \begin{tabular}[c]{@{}c@{}}0.1813 \\ ± 0.00014\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.24479 \\ ± 0.00012\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.09407 \\ ± 9e-05\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.07602 \\ ± 6e-05\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.01263 \\ ± 2e-05\end{tabular} \\
Coarse & iQMC & 0.15697    & 0.22319     & 0.08261      & 0.07097     & 0.0126 \\
\rowcolor[HTML]{EFEFEF} 
Fine & iQMC  & 0.18251    & 0.24507     & 0.09452      & 0.07652     & 0.01275 \\ \hline
\end{tabular}
\label{table:c5g7_fast}
\end{table}

==> tables/c5g7_results_thermal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{table}
\caption{Region averaged scalar flux from 2D-C5G7: groups 3-7 (slow)}
\centering
\begin{tabular}{|lcccccc|}
\hline
\textbf{Mesh} & \textbf{Method} & \textbf{I} & \textbf{II} & \textbf{III} & \textbf{IV} & \textbf{Moderator} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c}{\cellcolor[HTML]{EFEFEF}Coarse} &
  \begin{tabular}[c]{@{}c@{}}Monte Carlo\\  (Reference)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.11494 \\ ± 0.00012\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.11397 \\ ± 9e-05\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.04833 \\ ± 6e-05\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.0487 \\ ± 6e-05\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}0.037 \\ ± 6e-05\end{tabular} \\
Coarse        & iQMC            & 0.09848    & 0.10269     & 0.04242      & 0.04497     & 0.03551            \\
\rowcolor[HTML]{EFEFEF} 
Fine          & iQMC            & 0.11542    & 0.11403     & 0.04852      & 0.04891     & 0.03723            \\ \hline
\end{tabular}
\label{table:c5g7_slow}
\end{table}

==> tables/takeda1_error.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}
\centering
\label{table:takeda1_error}
\caption{Region averaged scalar flux relative error.}
\begin{tabular}{|llrrr|}
\hline
\multicolumn{1}{|c}{\textbf{N}} &
  \multicolumn{1}{c}{\textbf{Method}} &
  \multicolumn{1}{c}{\textbf{Core}} &
  \multicolumn{1}{c}{\textbf{Control Rod}} &
  \multicolumn{1}{c|}{\textbf{Moderator}} \\ \hline
  \rowcolor[HTML]{EFEFEF} 
$3.125\times 10^6$ & iQMC     &         &         &         \\
                    \rowcolor[HTML]{EFEFEF} 
                   & Constant & 0.0528 & 0.0367 & 0.0967 \\
                   \rowcolor[HTML]{EFEFEF} 
                   & Linear   & 0.1534 & 0.1604 & 0.1774 \\
                   \rowcolor[HTML]{EFEFEF} 
                   & Bilinear & 0.4003 & 0.4184 & 0.463 \\
                   
$3.125\times 10^7$ & iQMC     &        &        &         \\
                   & Constant & 0.0706 & 0.0559 & 0.1168  \\
                   & Linear   & 0.0051 & 0.0055 & 0.0051 \\
                   & Bilinear & 0.0073 & 0.0078 & 0.0078 \\ \hline
\end{tabular}
\end{table}

==> tables/takeda1_fom.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}
\centering
\label{table:takeda1_fom}
\caption{Region averaged scalar flux figure of Merit.}
\begin{tabular}{|llrrr|}
\hline
\multicolumn{1}{|c}{\textbf{N}} &
  \multicolumn{1}{c}{\textbf{Method}} &
  \multicolumn{1}{c}{\textbf{Core}} &
  \multicolumn{1}{c}{\textbf{Control Rod}} &
  \multicolumn{1}{c|}{\textbf{Moderator}} \\ \hline
  \rowcolor[HTML]{EFEFEF} 
$3.125\times 10^6$ & iQMC     &         &         &         \\
                    \rowcolor[HTML]{EFEFEF} 
                   & Constant & 0.0839 & 0.1209 & 0.0459 \\
                   \rowcolor[HTML]{EFEFEF} 
                   & Linear   & 0.0237 & 0.0227 & 0.0205 \\
                   \rowcolor[HTML]{EFEFEF} 
                   & Bilinear & 0.0079 & 0.0075 & 0.0068 \\
                   
$3.125\times 10^7$ & iQMC     &        &        &         \\
                   & Constant & 0.0385 & 0.0486 & 0.0233  \\
                   & Linear   & 0.3335 & 0.3069 & 0.334 \\
                   & Bilinear & 0.1736 & 0.1633 & 0.1625 \\ \hline
\end{tabular}
\end{table}

==> tables/takeda1_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}
\centering
\label{table:takeda1_results}
\caption{Region averaged scalar flux from Takeda-1 benchmark, integrated over energy}
\begin{tabular}{|llrrr|}
\hline
\multicolumn{1}{|c}{\textbf{N}} &
  \multicolumn{1}{c}{\textbf{Method}} &
  \multicolumn{1}{c}{\textbf{Core}} &
  \multicolumn{1}{c}{\textbf{Control Rod}} &
  \multicolumn{1}{c|}{\textbf{Moderator}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
$10^9$ &
  \begin{tabular}[c]{@{}l@{}}Monte Carlo\\ (Reference)\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}0.22884 \\ ± 2e-05\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}0.05653 \\ ± 1e-05\end{tabular} &
  \begin{tabular}[c]{@{}r@{}}0.20992 \\ ± 3e-05\end{tabular} \\
$3.125\times 10^6$ & iQMC     &         &         &         \\
                   & Constant & 0.21675 & 0.05445 & 0.18962 \\
                   & Linear   & 0.26395 & 0.06559 & 0.24716 \\
                   & Bilinear & 0.32045 & 0.08018 & 0.30711 \\
\rowcolor[HTML]{EFEFEF} 
$3.125\times 10^7$ & iQMC     &         &         &         \\
\rowcolor[HTML]{EFEFEF} 
                   & Constant & 0.21267 & 0.05337 & 0.1854  \\
\rowcolor[HTML]{EFEFEF} 
                   & Linear   & 0.23    & 0.05684 & 0.21098 \\
\rowcolor[HTML]{EFEFEF} 
                   & Bilinear & 0.23051 & 0.05697 & 0.21156 \\ \hline
\end{tabular}
\end{table}
